Building Anosov flows on 3-manifolds

We prove a result allowing to build (transitive or non-transitive) Anosov flows on 3-manifolds by gluing together filtrating neighborhoods of hyperbolic sets. We give several applications; for example: 1. we build a 3-manifold supporting both of a transitive Anosov vector field and a non-transitive Anosov vector field; 2. for any n, we build a 3-manifold M supporting at least n pairwise different Anosov vector fields; 3. we build transitive attractors with prescribed entrance foliation; in particular, we construct some incoherent transitive attractors; 4. we build a transitive Anosov vector field admitting infinitely many pairwise non-isotopic trans- verse tori.

==> structure.tex <==
\section{Spectrum like Decomposition}

\subsection{Periodic Saddle Basic Set in Seifert Manifold}
A similar definition can be found in \cite{BaFe}.
\begin{definition}
 A saddle basic set $\Lambda$ with  a filtrating neighborhood $N$ satisfying the following three conditions is called \emph{periodic},
    \begin{enumerate}
      \item $N$  is a Seifert manifold  with boundary;
      \item every boundary periodic orbit of $\Lambda$ is isotopic to a regular fiber of $N$;
      \item $W^s (\Lambda)$ and $W^u (\Lambda)$ can be expanded to two foliations in $N$ satisfying that the foliations transversely intersect $\partial N$.
    \end{enumerate}
\end{definition}


\begin{proposition}Let $N$ be a filtrating neighborhood of a saddle basic set $\Lambda$.
 The following five statements are equivalent.
\begin{enumerate}
  \item $W^s (\Lambda)$ and $W^u (\Lambda)$ can be expanded to two foliations in $N$ such that the foliations transversely intersect $\partial N$.
  \item $W^s (\Lambda)$ can be expanded to a foliation in $N$ such that the foliation  transversely intersect $\partial N$.
  \item $W^u (\Lambda)$ can be expanded to a foliation in $N$ such that the foliation  transversely intersect $\partial N$.
  \item $W^s (\Lambda) \cap \partial^{in} N$ can be expanded to a foliation in $\partial^{in} N$.
  \item $W^u (\Lambda) \cap \partial^{out} N$ can be expanded to a foliation in $\partial^{out} N$.
\end{enumerate}
\end{proposition}

\begin{proof}
We only need to prove that  condition $1$ can be deduced by condition $5$. Let us explain the  reason. It is obviously that condition $1$ deduces condition $3$ and condition $5$, and condition $3$ deduces condition $5$.
So if condition $5$ deduces condition $1$, then condition $1$, condition $3$ and condition $5$ are equivalent. For symmetrical reason, if condition $5$ can deduce condition $1$, then condition $4$ also can deduce condition $1$. Therefore, similarly, condition $2$, condition $4$ and condition $5$ also are equivalent.

Now we focus on proving that condition $5$ deduces condition $1$. By Theorem 5.3 and the tool similar to the construction in the proof of Theorem 5.3, we can find a attracting plug $V$ with transitive maximal invariant set $A$ such that we can glue $\partial^{in} V$ to $\partial^{out} N$ satisfying $W^s (A)$
transversely intersects $W^u (\Lambda)$. We call the new compact 3-manifold $W$ with flow $\psi_t$. We define by $\Lambda_0$ the maximal invariant set of $\psi_t$. Actually $\Lambda_0 = W^s (\Lambda) \cup A$. $W^s (\Lambda_0)$ gives $W$ a 2 dimensional foliation which is transverse to $\partial^{in} (\Lambda_0)$. Obviously, in $W$, the lamination $W^s(\Lambda)$ is a sub-foliation of $W^s (\Lambda_0)$. Furthermore, $W^s(\Lambda) \cap \partial^{in} (W)$ can be extended to the foliation $W^s(\Lambda_0) \cap \partial^{in} (W)$.

$W$ is a attracting plug, by Theorem 5.3 and the tool similar to the construction in the proof of Theorem 5.3, we can build a repelling plug $U$ with a flow $\phi_t$ the maximal invariant set $\Lambda_1$
and a diffeomorphism $f:\partial^{out} U \rightarrow \partial^{in} W$ such that $f(W^u (\Lambda_1))$ is transverse to $W^s (\Lambda_0)$. Then by Theorem 1.1, the flow $\varphi_t$ induced by $\psi_t$ and $\phi_t$ by the gluing $U \coprod W /f $ is an Anosov flow. Notice that  for $\varphi_t$, $W^s (M)$ and $W^u (M)$ are two transversely intersected foliations. Moveover, $W^s (\Lambda)$ is a sub-foliation of $W^s (M)$ and $W^u (\Lambda)$ is a sub-foliation of $W^u (M)$. Therefore, we have that $W^s (\Lambda)$ and $W^u (\Lambda)$ satisfy condition $1$.
\end{proof}

\begin{lemma}
Let $\Lambda$ be a periodic saddle basic set with a Seifert filtrating neighborhood $N$. Then $W^s (\Lambda)$ can be expanded to a foliation
$\mathcal{F}$ such that there doesn't exist any compact leaf in $\mathcal{F}-W^s (\Lambda)$.
\end{lemma}
\begin{proof}

   In the same way with the proof of Proposition 5.2, we can extend $W^s {\Lambda}$ to a foliation $\mathcal{F}_0$ with finitely many compact leaves or without any compact leaf. If $\mathcal{F}_0$ doesn't have any compact leaf, we suppose $\mathcal{F}=\mathcal{F}_0$. The following we deal with the case that $\mathcal{F}_0$ admits finitely many compact leaves.

   There exist $n$ open annuli $A_1, ..., A_n \subset \partial^+ {N}$ which satisfy that their boundary is composed of  closed leaves in $\partial^+ N - W^s {\Lambda}$ and
       they are disjoint with $W^s {\Lambda}$. Denote $\mathcal{F}_0 \cap \partial^+ N$ by $\mathcal{F}_0'$.
   In an open annulus, for example, $A_1$, we choose a smaller open annulus $A_1' \subset A_1$ such that $A_1'$ is homotopic equivalent to $A_1$ and $\partial A_1'$ ia very close to $\partial A_1$.  By natural way,  we can  build a foliation $\mathcal{F}_1'$ on $\partial^+ N$ such that $\mathcal{F}_1' = \mathcal{F}_0'$ in the out side of $A_1'$ and there doesn't exist a closed leaf in $A_1$.
 $\mathcal{F}_1'$ can be extended to a foliation $\mathcal{F}_1$ with fewer compact leaves. This process goes on until we construct $\mathcal{F}_m$ ($1\leq m\leq n$) which doesn't contain any compact leaf in $\mathcal{F}_m-W^s (\Lambda)$. Now we define $\mathcal{F}= \mathcal{F}_m$. It is easy to check that $W^s (\Lambda)$ is a sub-foliation of $\mathcal{F}$ and $\mathcal{F}$ doesn't contain any compact leaf.
\end{proof}

The following useful lemma was used in Brunella's paper \cite{Br}, now we state it exactly and give a strict proof.

\begin{lemma}
  Let $\Lambda$ be a nontrivial saddle basic set with filtrating neighborhood $N$. Then for every periodic orbit $\gamma\in \Lambda$, the fundamental group of the double of the weak stable manifold $W^s (\gamma) \cap N$, $L$ has infinitely many generators. Where $L$ is constructed by gluing  two $W^s (\gamma)$ along $W^s (\gamma) \cap \partial N$ by identity map.
\end{lemma}

\begin{proof}
Let $x$ be a point in $\gamma$ and $W^{ss}(x)$ be the strong stable manifold of $x$. Suppose that $f$ is the first return map of the flow restricted to $W^{ss}(x)$. Obviously $f$ is an attracting map with exactly one fixed point $x$.   By the structure of dimension 1 saddle basic sets, $\Lambda \cap W^{ss}(x)$ is a cantor set and for a fundamental domain $D(f)$ of $f$ which is sufficiently close to $x$, $D(f)-\Lambda$ consists in infinitely many
open intervals. Since $D(f)$ is a fundamental domain of $f$, this means each two intervals of  $D(f)-\Lambda$ are in two different connected components of $W^{s}(\gamma)-\Lambda$. Therefore, $W^{s}(\gamma)-\Lambda$ consists of infinitely many connected components. Since $\Lambda$ is
the maximal invariant set of the flow in $N$, for each connected component $C$ of $W^{s}(\gamma)-\Lambda$, $C \cap \partial^{in} N \neq \emptyset$. There exists an open interval $l \subset C \cap \partial^{in} N \neq \emptyset$ which converges to the  boundary of $C$ similar to the behavior that a normal leaf of a Reeb annulus  converges to two compact leaves of the Reeb annulus. By this reason and the fact that $W^{s}(\gamma)-\Lambda$ consists of infinitely many connected components, the double of the weak stable manifold $W^s (\gamma)$, $L$ is a surface with infinitely many cusps. Therefore, $\pi_1 (L)$ has infinitely many generators.
\end{proof}

  There is a classic theorem in low dimensional topology: every incompressible surface in a Seifert manifold $M$ is isotopic to a surface which is either vertical, i.e., a union of regular fibers, or horizontal, i.e., transverse to all fibers (see \cite{Ha}). The following theorem of Brittenham  [Bri]  generalizes it to a more general case: essential lamination, in particular, taut foliation. Since we only use the theorem under the condition taut foliation and  to ovoid defining essential lamination,  we state the theorem  as follows.

\begin{theorem}
Let $M$ be a Seifert manifold with a Seifert fiber over an orbifold
$\Sigma$, and let $\mathcal{F}$ be a taut foliation of $M$. Then there is a lamination  $\mathcal{L}$ which is a sub-foliation of $\mathcal{F}$
up to the isotopy, every leaf of $\mathcal{L}$ is either vertical (its leaves are foliated by fibers of $M$)  or horizontal (its leaves are everywhere transverse to the circle fibers of $M$).
\end{theorem}

\begin{lemma}
If a leaf $L$ of a lamination in a Seifert manifold $M$ is horizontal, then every simple closed curve in $L$ is not isotopic to  a regular fiber.
\end{lemma}

\begin{proof}
Otherwise, there exists a simple closed curve $c$ in $L$ which is isotopic to a regular fiber. Let $\Sigma$ be the orbifold corresponding to the regular fiber and $\pi: M\rightarrow \Sigma$ be the natural projection map. Since $c$ is isotopic to the regular fiber, $c$ is essential in $L$.
$\pi: L\rightarrow \Sigma$ is a branched covering, so $\pi (c)$ is an essential simple closed curve in $\Sigma$. Therefore, $T=\pi^{-1} (\pi (c))$
is a incompressible torus in $M$. Obviously, $c$ and a regular fiber are two nonparallel simple closed curves in $T$. $T$ is incompressible, so $c$
can't be isotopic to a regular fiber. It is a contradiction.
\end{proof}



Now, we can state the main theorem in this section.

\begin{theorem}
 Let $\Lambda$ be a periodic saddle basic set in a Seifert manifold $N$, then $\Lambda$ is an isolated saddle periodic orbit.
\end{theorem}

\begin{proof}
 By Lemma 6.3, we can expand $W^s (\Lambda)$ to a foliation $\mathcal{F}$ which is transverse to $\partial N$ and $\mathcal{F}$ doesn't have a compact leaf in $N$.  Now we define double $N$, $W$ which is  constructed by gluing  two $N$ along $\partial N$ by identity map. Obviously $W$ still is a Seifert manifold. $\mathcal{F}$ provides a natural foliation $\overline{\mathcal{F}}$ on $W$.

Suppose $\Lambda$ is a nontrivial basic set, by the construction of $\overline{\mathcal{F}}$ and Lemma 6.4, each leaf of $\overline{\mathcal{F}}$ is noncompact.
 Therefore $\overline{\mathcal{F}}$ is taut.  By Theorem 6.5, there exists a lamination  $\mathcal{L}  \subset \overline{\mathcal{F}}$ is either vertical or horizontal.
  By the construction of $\overline{\mathcal{F}}$ and the compact of $\mathcal{L}$, $\mathcal{L} \cap \partial N$ contains some simple closed curves which are isotopic to a regular fiber.
 Lemma 6.6 forbids  $\mathcal{L}$ to be horizontal. So it is only possible that $\mathcal{L}$ is vertical. Each leaf in $\mathcal{L}$ is foliated by some regular fibers, so every leaf has to be homeomorphic to one of torus, annulus, Klein bottle and Mobius band.
But Lemma 6.4 tell us that there exits a leaf $L$ in $\mathcal{L}$ such that $\pi_1 (L)$ is infinitely generated, therefore $L$ isn't homeomorphic to one of torus, annulus, Klein bottle and Mobius band. It is a contradiction. Therefore, $\Lambda$ has to be an isolated saddle periodic orbit.
\end{proof}

A filtrating neighborhood of an isolated saddle periodic orbit is called a fattened round 1-handle by J. Morgan \cite{Mo} to discuss nonsingular Morse-Smale flows on 3-manifolds. Actually, he classified all such kind of filtrating neighborhoods with tori boundary up to  topological equivalence. For us, by Theorem 6.7,
a filtrating neighborhood of a periodic saddle basic set is exactly a filtrating neighborhood of an isolated saddle periodic orbit whose stable and unstable laminations can be extended to  two foliations of the filtrating neighborhood. By \cite{Mo}, such filtrating neighborhoods can be described as follows.

\begin{proposition}
Let $\Lambda$ be a periodic saddle basic set in Seifert manifold $N$. Then, $\Lambda=\gamma$ where $\gamma$ is a saddle periodic orbit, and up to topological equivalence, $(N,\Lambda)$ is topological equivalence to one of  the following four cases.
\begin{enumerate}
  \item $V_1$ is homeomorphic to $\Sigma_0^3 \times S^1$ here $\Sigma_0^3$ is a 2-sphere with three punctures and $\partial \Sigma_0^3$ consists of three simple closed curves $c_1$, $c_2$ and $c_3$. $\partial^{in} V_1 = c_1 \times S^1$ and $\partial^{out} V_1 =c_2 \times S^1 \cup c_3\times S^1$. $W^s (\gamma)\cap \partial^{in} V_1$ consists of two parallel simple closed curves with the same orientation which are isotopic to $\{\ast\} \times S^1$. $W^u (\gamma)\cap \partial^{out} V_1$ consists of two parallel simple closed curves in $c_2 \times S^1$ and $c_3 \times S^1$, respectively. Furthermore, both of these two simple closed curves are isotopic to $\{\ast\} \times S^1$.
  \item $V_2$ is the first case with converse direction of the flow.
  \item $V_3$ is homeomorphic to twisted $S^1$ bundle over punctured Mobius band. Each of $\partial^{in} V_3$ and $\partial^{out} V_3$ is a torus.
  $W^s (\gamma)\cap \partial^{in} V_3$ consists of two parallel simple closed curves with the converse orientation which are isotopic to $\{\ast\} \times S^1$. It is similar to $W^u (\gamma)\cap \partial^{in} V_3$.

  \item $V_4$ is homeomorphic to $U-U_0$ here $U$ is a solid torus and $U_0$ is a solid torus in $U$ such that the core of $U_0$ is a closed 2 braid of $U$. $\partial^{in} V_4 = \partial U_0$ and $\partial^{out}V_4 =\partial U$. $\gamma$ is  isotopic to the core of $V_4$.  $W^s \cap \partial^{in} V_4$ is a  simple closed curve in $\partial U_0$ which is isotopic to the core of $U_0$.  $W^u \cap \partial^{in} V_4$ is a simple closed curve in $\partial U$ which is a $(2,1)$ curve in $\partial U$. Where $(1,0)$ is isotopic to the core of $U$ and $(0,1)$ is a meridian of $U$.
\end{enumerate}
\end{proposition}

\begin{remark}
\begin{enumerate}
  \item The Anosov flow which we constructed in the proof of Theorem 4.1  can be regarded as gluing two filtrating neighborhoods of (1) in the proposition and  two filtrating neighborhoods of (2) in the proposition   suitably.
  \item The  Anosov flow of \cite{BoLa1} can be regarded as gluing a filtrating neighborhood of (3) in the proposition suitably.
\end{enumerate}
\end{remark}


\subsection{Canonical Basic Sets Decomposition}
\begin{definition}
Let $N$ be a compact three manifold and $X$ be a smooth flow on $N$. $\partial N= \partial^{+} N \cup_c \partial^{-} N$ here $c$ is composed of  some pairwise disjoint simple closed curves on $\partial N$ and $X$ is transverse inside to $N$ along the interior of $\partial^{+} N$ and outside to $N$ along the interior of $\partial^{-} N$. We call $(N,X)$ satisfies the \emph{corner condition} if there exists a neighborhood $N(c)$ of $c$ in $N$ such that
every flowline in $N(c)$ of $X$ disjoint with $c$ is an arc whose two ends are in $\partial^{+} N$ and $\partial^{-} N$ correspondingly.
\end{definition}


\begin{lemma}
Let $X$ be an Anosov flow on a closed orientable three manifold $M$ and $N\subset M$ be a compact three manifold. If $(N,X|_N)$ satisfies the corner condition and one of the following conditions,
\begin{enumerate}
  \item $N$ is homeomorphic to $T^2 \times I$ and $X|_N$ is transverse to $\partial N$;
  \item $N$ is homeomorphic to a 3-ball and $\partial N= D^1 \cup_c D^2$, here $D^1$ and $D^2$ are two disks and $c=\partial D^1 =\partial D^2 \subset \partial N$. Moreover, $X$ is transverse inside to $N$ along the interior of $D^1$ and outside to $N$ along the interior of $D^2$;
  \item $N$ is homeomorphic to $D^2 \times S^1$ by $f$, here $D^2=\{\rho e^{i\theta}| \rho \in [0,1], \theta\in [0,2\pi]\}$, $X|_N$ is transverse inside to $N$ along the interior of $l_1 \times S^1$ and outside to $N$ along the interior of $l_2 \times S^1$, here $l_1=\{e^{i\theta}| \theta \in [0,\pi]\}$ and $l_2=\{e^{i\theta}| \theta \in [\pi,2\pi]\}$;
\end{enumerate}
then the invariant set of $X|_N$ is empty.
\end{lemma}

\begin{proof}
If $(N,X|_N)$ satisfies condition 1, suppose the maximal invariant set of $X|_N$ is not empty. By Lyapunov theory, we can find finitely many of pairwise disjoint transverse tori $T_1, ..., T_n \subset N$  which cut $N$
to $m$ compact components $N_1, ..., N_m$ which satisfy that the maximal invariant set of each $N_j$ ($j\in \{1,...,m\}$) is a saddle basic set $\Lambda_j$. Notice that $T_i$ ($i\in \{1,...,n\}$) is incompressible in $M$ (see \cite{Br} or Corollary 2.2 in \cite{Fe}), therefore each $T_i$ is incompressible in $N$. Moveover, $T_i$ has to be isotopic to $T^2 \times \{0\}$ since $N$ is homeomorphic to $T^2 \times I$. This fact tell us $N_j$ is homeomorphic to $T^2 \times I$. Because of the topology of $T^2 \times I$ and $X$ is an Anosov flow on $M$, $\Lambda_j$ is a periodic saddle basic set in $N_0$. By Theorem 5.7, $\Lambda$ is an isolated saddle periodic orbit. By Proposition 5.8, $N_j$ isn't homeomorphic to $T^2 \times I$. It is a contradiction. 1 is proved.

If $(N,X|_N)$ satisfies condition 2, denote $\Lambda=\lim_{t\rightarrow +\infty} \cap X_{[-t,t]} (N)$, i.e., the maximal invariant set of $X|N$. We suppose that $\Lambda\neq \emptyset$. Since $X$ is an Anosov flow on $M$,
$\Lambda$ is a  hyperbolic invariant set. $X$ satisfies the corner condition, $W^s(\Lambda)\cap D^1$  is in the interior of $D^1$. Since there exists a stable boundary periodic orbit in $\Lambda$, there exists a closed leaf $L$ in  the lamination $W^s(\Lambda)\cap D^1$ which bounds a disc $D_1 '$ in $D^1$.  $W^s(\Lambda)\cap D^1$ can never be extended to a foliation in $D_1'$. But $\{W^s (x)\cup D_1'| x\in M\}$ gives a foliation on $D_1'$. But $D_1'$ is homeomorphic to a disk, by Poincare-Hopf index theorem, $D_1'$ can't admit a 1 dimensional foliation such that  $\partial D_1'$ is a leaf. Therefore, the case in the supposition can't appear and $\Lambda=\emptyset$. 2 is proved.

If $(N,X|_N)$ satisfies condition 3, let $N_A=A\times I$ be a thickened annulus with vector field $Y$ given by $\frac{\partial}{\partial t}$ , here $A$ is an annulus and $I=\{t|0\leq t\leq1\}$. Set $c_1 =\{1\} \times S^1$ and $c_2= \{-1\} \times S^1$ which are two simple closed curves in $\partial N$. Since $(N,X|N)$ satisfies the corner condition, we cut a suitable small neighborhood $N(c_1)\sqcup N(c_2)$ of $c_1$ and $c_2$ in $N$ and glue $N_A$ to $\overline{N-N(c_1)\sqcup N(c_2)}$ along the flowlines of  $\partial A \times I$ and the place we cut in  $\partial \overline{N-N(c_1)\sqcup N(c_2)}$. After these surgeries, we obtain a new manifold $W$ with flow $Y$.  If we choose $N(c_1)$ and $N(c_2)$ suitably, $\Lambda$ can be the maximal invariant set of $(W,Y)$. Obviously $W$ is homeomorphic to $T^2 \times [0,1]$.   A transverse torus $T\subset W$ either is disjoint with $N_A$ or intersects $N_A$. If $T$ is disjoint with $N_A$, then $T\subset N$, therefore $T$  is incompressible in $W$. If $T$ intersects $N_A$, by the structure of $Y$, it is easy to show that $T$ is isotopic to $\partial^+ W$. Therefore, $T$ is incompressible in $W$.
Now, we can do the same argument as the first case to finish the proof of 3.
\end{proof}

Let $X$ be an Anosov flow on a closed orientable three manifold $M$ and $N\subset M$ be a compact three manifold. If $(N,X|_N)$ can be parameterized as the third case in the above lemma, we call $(N,X|_N)$ a \emph{solid torus with two cusps}. Let $\tau=\{T_1, ...,T_n\}$ be an incompressible, transversely intersected tori set in an irreducible three manifold $M$.
We define $Ord (\tau)= (tr(\tau),in(\tau),es(\tau))$ here $tr(\tau)$ is the number of the triple intersection points in $\tau$, $in(\tau)$
is the number of inessential intersection simple closed curves between two tori in $\tau$ and $es(\tau)$ is the number of essential intersection
simple closed curves between two tori in $\tau$. This order naturally gives an ... order of  a transverse tori set.    $T_1,  ..., T_n$  are in \emph{minimal position} if $tr(\tau)=0$, $in(\tau)=0$ and there doesn't exist a solid torus with two cusps in $M-(T_1 \cup ... \cup T_n)$. We call $T_1,...,T_n$ are \emph{flow-isotopic} to $T_1',...,T_n'$ if each $T_i$ ($i\in \{1,...,n\}$)is isotopic to $T_i'$ along flowline of $X$.

\begin{remark}
Similar to the case of simple closed curves in surfaces \cite{FaMa}.  $\tau=\{T_1, ..., T_n\}$ are in minimal position also means that $es(\tau)$
is minimal among  $es(\tau')$ for all $\tau'$ such that $\tau' = \{T_1' ,..., T_n'\}$ and $T_i'$ ($i=1,...,n$) is isotopic to $T_i$. Its proof is similar to the case of simple closed curves in surfaces. Since actually we don't use this property, so we omit its proof here.
\end{remark}



The following theorem is a standard theorem of low dimensional topology, see \cite{Ha}.

\begin{theorem}
Let $T$ be an incompressible torus in an irreducible three manifold $M$, then $T$ is isotopic to either a  JSJ torus or a vertical torus in a Seifert piece of M. Where a vertical torus is an incompressible torus which is foliated by some regular fibers of the Seifert piece.
\end{theorem}

This theorem tell us that there always exist tori  $T_1', ..., T_n'$ which satisfies the following conditions.
\begin{itemize}
  \item $T_i'$ ($i=1,...,n$) is isotopic to $T_i$.
  \item $T_1',...,T_n'$ are in minimal position.
\end{itemize}

\begin{lemma}
Let $X$ be an Anosov vector field on a closed orientable three manifold  $M$ and $\tau=\{T_1, ...,T_k\}$ be a pairwise disjoint, nonparallel transverse tori set in $M$. For a given transverse torus $T_{k+1}$, $T_{k+1}$ can be flow-isotopic to $T_{k+1}'$ such that $T_1, ...,T_k,T_{k+1}'$ are in minimal position.
\end{lemma}
\begin{proof}

 Set $\Gamma=\{\{T_1, ..., T_k, T_{k+1}^0\}\}$ here $T_{k+1}^0$ is flow-isotopic to $T_{k+1}$. Suppose $\tau'= \{T_1,...,T_k, T_{k+1}'\} \in \Gamma$ satisfies that $\tau'$ is minimal among all $\tau \in \Gamma$ under the ... order. $Ord (\tau')= (tr(\tau'),in(\tau'),es(\tau'))$. Obviously $tr(\tau')=0$.

 If $in(\tau') \neq 0$, Then there exists $T_1$ (without confusion) and  an inessential simple closed curve $c\subset T_1\cap T_{k+1}'$ which bounds disks $D_1 \subset T_1^1$ and $D_{k+1} \subset T_{k+1}'$. We can suppose that they satisfies that $D_1 \cup D_{k+1}$ bounds a 3-ball $B \subset M$ and the interior of $B$ doesn't intersect with $\tau'$. The fact that such a simple closed curve exists is because of both of $T_1$ and $T_{k+1}'$ are incompressible and $M$ is an irreducible 3-manifold.


\begin{figure}[htp]
\begin{center}
  \includegraphics[totalheight=5.2cm]{figure1.eps}\\
  \caption{}\label{figure1}
  \end{center}
\end{figure}

 The flow $X$ is transverse inside to $B$ along  the interior of one of $D_1$ and $D_{k+1}$ and is transverse outside to $B$ along the interior of the other. Without confusion, we suppose that $X$ is transverse inside to $B$ along the interior of $D_{k+1}$, see Figure.. . Now we can choose $D_{k+1}'$ and $D_1'$ as follows. We choose an annulus $A\subset T_{k+1}'$ in a small neighborhood of $B$ such that $A\cap D_{k+1} =c$ and $\partial A - c$ bounds a disk $D_1'$ in $M$ such that $X$ is transverse to the interior of $D_1'$ and $D_1 \cup A \cup D_1'$ bounds a 3-ball $B_0$ in $M$, see Figure.. . Set $B_1 = B\cup B_0$ which also is a 3-ball in $M$. $X$ transverse into $B_1$ along the interior of $D_{k+1}'$  and transverse outside to $B_1$ along the interior of $D_1'$.
 By (2) of Lemma 6.2 , we can push $D_{k+1}'$ to $D_1'$ along flowline of $X$.
Where $D_{k+1}'$ and $D_1'$ are two disks (see (1) of Figure 1) which satisfies the following conditions.
\begin{itemize}
 \item $D_{k+1}\subset D_{k+1}' \subset T_{k+1}'$ and $D_{k+1}'$ is in a small neighborhood
of $D_{k+1}$.
   \item $D_1'$ is transverse to the flowline of $X$ and is in a small neighborhood of $T_1^1$, $\partial D_1' =\partial D_{k+1}'$ and $D_1' \cap (T_1 \cup...\cup T_k) =\emptyset$.
\end{itemize}
 Set $T_{k+1}^2 =(T_{k+1}' -D_{k+1}')\cup D_1'$. Then $\tau^2=\{T_1,...,T_k, T_{k+1}^2\} \in \Gamma$,  but
 $Ord(\tau^2)< Ord(\tau')$.  It is a contradiction with the supposition of $\tau'$.


 If $in(\tau')=0$ and there exists a solid torus with two cusps in $M-(T_1 \cup ... \cup T_k \cup T_{k+1}')$. The boundary of the solid torus is belong to $T_i \cup T_{k+1}'$ for some $i \in \{1,...,k\}$. Then, by (3) of Lemma 6.2, similar to the case $in(\tau')\neq 0$, we can push $T_{k+1}'$ to $T_{k+1}^2$ along the flowlines of $X$ such that $Ord(\tau^2)<Ord(\tau')$ here $\tau^2 =\{T_1,...,T_k, T_{k+1}^2\}$
      (see (2) of Figure 1).
      It conflicts our supposition.


 In summary, $\tau'$ is in minimal position.
\end{proof}






Now we introduce a little bit train track theory, which provides a suitable language for the following part.  More details about train track theory can be found in \cite{PeHa}.

\begin{definition}
A \emph{train track} $\tau$ on $\Sigma$ is an embedded 1-complex  whose
edges (called \emph{branches}) are smooth arcs with well-defined tangent vectors at the
endpoints. At any vertex (called a \emph{switch}) the incident edges are mutually tangent.
\end{definition}

\begin{remark}
A normal definition of train track always includes some restrictions of the topology of each connected component of $\Sigma - \tau$. But for our purpose, the above definition is enough. It should be noted that the following properties about train track is still correct under our definition, see .
\end{remark}

\begin{definition}
Let $\tau$ be a train track on an orbifold $\Sigma$.
A \emph{recurrent circle} $C\subset \tau$ is an immersed circle $F(e^{i\theta})| \theta \in \mathcal{R}$ in $\tau$ here $F(e^{i\theta}): \mathcal{R} \rightarrow \tau$ is a smooth map. $\tau$  is called \emph{recurrent} if for each  point $P\in \tau$, there exits a recurrent circle which passes through $P$. A \emph{measure} on $\tau$ is a nonnegative weight function $\mu$ on
the branches on $\tau$ satisfying the switch condition: For every switch $v$ of $\tau$, the sum
of the weights of all incoming branches at $v$ is equivalent to the sum
of the weights of all outgoing branches at $v$.
\end{definition}

\begin{definition}
Let $\tau$ be a train track on an orbifold $\Sigma$. A \emph{support} of $\tau$, $Supp(\tau)$ is a  neighborhood of $\tau$ with an oriented line bundle. A \emph{transverse multi-curve} in $\Sigma$ is the union of a finite collection of disjoint
simple closed curves in $Supp(\tau)$ which are transverse to the oriented line bundle over $Supp(\tau)$.
\end{definition}

\begin{proposition}
Let $\tau$ be a train track on an orbifold $\Sigma$ and $Supp(\tau)$ be a support of $\tau$.   The following three statements are equivalent.
\begin{enumerate}
  \item $\tau$ is recurrent.
  \item There exists a positive measure $\mu$  on $\tau$. Where a positive measure $\mu$ is positive on every branch.
  \item There exists a transverse multi-curve which intersects line fiber of $Supp(\tau)$.
\end{enumerate}
\end{proposition}










\begin{lemma}
Let $X$ be an Anosov vector field on a closed orientable three manifold  $M$. Suppose that  $T_1, ...,T_k, T_{k+1}$ are $k+1$ transverse tori of $X$ such that  they are in minimal position and $T_1, ...,T_k$ are pairwise disjoint and nonparallel. Then the nonwandering set of $X|_{M-(T_1 \cup ...\cup T_k \cup T_{k+1})}$ is composed of finitely many  basic sets $\Lambda_1, ..., \Lambda_m$. Furthermore, there exists  pairwise disjoint and nonparallel transverse tori $T_1' ,..., T_n'$ such that they cut $M$ to $M_1,..., M_m$ such that each $M_i$ ($i\in \{1,...,m\}$) is a filtrating neighborhood of $\Lambda_i$.
\end{lemma}
\begin{proof}
  Suppose $M- T_1 \cup ... \cup T_k \cup T_{k+1}$ is composed of $s$ connected components $M_1, ..., M_s$.   For each $i\in \{1,...,s\}$, it is easy to check that  the nonwandering set of $X|_{M_i}$, $\Omega (X, M_i)$ is a hyperbolic compact set. Furthermore, by shadowing lemma, the periodic orbits in $X|_{M_i}$ is dense in $\Omega (X, M_i)$. Therefore, $X|_{M_i}$ is an Axiom A system. By Spectrum decomposition Theorem, $\Omega (X, M_i)$ is  composed of  finitely many basic sets. Then the nonwandering set of $X|_{M-(T_1 \cup ...\cup T_k \cup T_{k+1})}$ is composed of finitely many  basic sets. We denote these basic sets $\Lambda_1, ..., \Lambda_m$.

  \begin{figure}[htp]
\begin{center}
  \includegraphics[totalheight=4.3cm]{figure2.eps}\\
  \caption{}\label{figure2}
  \end{center}
\end{figure}



  Let $X$ be an Anosov vector field on a closed orientable three manifold  $M$. Suppose that  $T_1, ...,T_k, T_{k+1}$ are $k+1$ transverse tori of $X$ such that  they are in minimal position and $T_1, ...,T_k$ are pairwise disjoint and nonparallel. For simplify, we suppose that $M$ is a Seifert manifold. Set $\mathcal{T}=T_1 \cup ... \cup T_k \cup T_{k+1}$ which is a 2-complex in $M$. Then there always exists a small neighborhood of $\mathcal{T}$, $N(\mathcal{T})$ can be parameterized by a homeomorphism $F: (\Sigma_0 \times S^1, G_0 \times S^1 ) \rightarrow (N(\mathcal{T}), \mathcal{T})$  preserving flowlines.
Where $(\Sigma_0, G_0)$ is a compact surface, 1-complex pair which  is composed of some local charts in Figure.. $\Sigma_0$ is endowed with a vector field.  In Figure .. , $A$ and $B$ are two cusp points, the center is the local chart of $G_0$. Figure .. is a global example.

Since $M$ is a Seifert manifold and for a given $P_0 \in \Sigma_0$, $F(\{P_0\} \times S^1)$ is isotopic to a normal fiber of $M$, we can extend the circle foliation on $N(\mathcal{T})=F(\Sigma_0 \times S^1)$, $\mathcal{F}_0=\{ \{P\} \times S^1 | P \in \Sigma_0 \} $ to a Seifert fiber structure $\pi: M\rightarrow \Sigma$ on $M$. Where $\Sigma$ is the orbifold and $\pi$ is the projective map corresponding to the Seifert fiber structure.
Without confusion, we can regard $\pi(N)=\pi \circ F(\Sigma_0 \times S^1)$ as $\Sigma_0$ itself. This means that $\Sigma_0 \subset \Sigma$ is still endowed with the original vector field, cusps and the core $G_0$. The key to understand such parameters just is to regard $\Sigma_0 \subset \Sigma$ as a normal cross section, $F(\Sigma_0 \times \{Q\})\subset N(\mathcal{T})$ here $Q\in S^1$.

Now we  build a train track $\tau$ on $\Sigma$. $\tau \subset \Sigma_0$ and in each local chart, it is shown in Figure .. .  Figure .. is the  global example corresponding the example in Figure .. .  Naturally, $\Sigma_0$ is a support of $\tau$.
$\tau$ is automatically recurrent. Actually, we can endow $\tau$ with positive integers $\mu$ as follows. For the edges in a local chart as Figure .. shows, $\mu(a)=\mu(b)=\mu(c)=\mu(d)=1$ and $\mu(e)=2$. By Proposition .., the measure $\mu$ gives a transverse multi-curve which intersects each line fiber of $\Sigma_0$. Actually, we can understand the transverse multi-curve directly. The multi-curve is transverse to  each band of $\Sigma_0$ exactly once and in the crossing of $\Sigma_0$,  locally it is as  Figure .. shows. We suppose that the transverse multi-curve is $\mathcal{C}=\{C_1,...,C_{r_0}\}$. We suppose that $T_i^0=\pi^{-1} (C_i)$ ($i=1,...,r_0$) which is a torus in $M$. It is easy to check that $T_1^0 ,..., T_{r_0}^0$ are  pairwise disjoint , nonparallel and transverse to $X$. Moreover, since $\mathcal{C}$ intersects the flowline in $\Sigma_0$, $T_1^0 \cup ... \cup T_{r_0}^0 $ intersects each flowline in $N(\mathcal{T})$.

\begin{figure}[htp]
\begin{center}
  \includegraphics[totalheight=3.6cm]{figure3.eps}\\
  \caption{}\label{figure3}
  \end{center}
\end{figure}

Suppose $M- T_1^0 \cup ... \cup T_{r_0}^0$ is composed of $m_0$ connected components $M_1', ..., M_{m_0}'$ and $\Omega (X, M_i')$ ($i=1,...,m_0$) is the nonwandering set of $X|_{M_i'}$.    Since $T_1' \cup ... \cup T_{r_0}' $ intersects each flowline in $N(\mathcal{T})$ and each $T_i' \subset N(\mathcal{T})$ ($i=1,...,r_0$), $\Omega(X, M_1)\cup ...\cup \Omega(X, M_m) =\Omega(X, M_1')\cup ...\cup \Omega(X, M_s')=\Lambda_1 \cup... \cup  \Lambda_m$ (every new nonwandering orbit has to pass through $N(\mathcal{T})$). Also notice that $X$ is transverse to each connected component of $\partial M_i^0$,  we can use Lyapunov theory to extend $T_1^0, ..., T_{r_0}^0$ to $T_1^0, ..., T_{r_0}^0, ..., T_r^0$ which satisfies the following conditions.
\begin{enumerate}
  \item $T_1^0, ..., T_{r_0}^0, ..., T_r^0$ are pairwise disjoint, nonparallel and transverse to $X$.
  \item $T_1^0, ..., T_{r_0}^0, ..., T_r^0$ cut $M$ to $M_1^0,..., M_{m_0}^0$ such that each $\Lambda_i$ ($i=1,...,m$)  is in some $M_j^0$ ($j\in \{1,...,m_0\}$) and each $M_j^0$ contains at most 1 basic set.
\end{enumerate}

If $T_i^0$ is parallel to $T_j^0$ ($i\neq j$), we cancel one of $T_i^0$ and $T_j^0$ in $\{T_1^0, ..., T_{r_0}^0, ..., T_r^0\}$. We do such cancelations in $\{T_1^0, ..., T_{r_0}^0, ..., T_r^0\}$ such that the left tori is $\{T_1', ... T_n'\}\subset \{T_1^0, ..., T_{r_0}^0, ..., T_r^0\}$ which don't exist parallel tori. cut $M$ to $M_1,..., M_p$. By (2) of Lemma 6.2 and the property of $T_1^0, ..., T_{r_0}^0, ..., T_r^0$, it is easy to check that each $M_i$ ($i=1,...,p$) is exactly a filtrating neighborhood of $\Lambda_j$ for some $j\in\{1,...,m\}$. Therefore, $p=m$ and the lemma is proved.
\end{proof}



\begin{proof}[Proof of Theorem~\ref{t.decomposition}]
 We suppose that, for every  maximal nonparallel, pairwise disjoint transverse tori $T_1, ..., T_n$ which cut   $M$ to $M_1, ..., M_m$ and the maximal invariant set of $X|M_i$ is denoted by $\Lambda_i$ (obviously each $\Lambda_i$ is a basic set), there exists a transverse torus $\Sigma$ which satisfies $\Sigma \cap (\Lambda_1 \sqcup ... \sqcup \Lambda_n) \neq \emptyset$.

In the following we will play a game to find a contradiction under the assumption above.

  At first, we choose maximal nonparallel, pairwise disjoint, transverse tori $T_1^0, ..., T_{n_0}^0$ which cut   $M$ to $M_1^0, ..., M_{m_0}^0$ and the maximal invariant set of $X|M_i^0$ ($i\in \{1,...,m_0\}$) is denoted by $\Lambda_i^0$. There exists a transverse torus $\Sigma^0$ which satisfies $\Sigma^0 \cap \Lambda_{s_0}^0 \neq \emptyset$ for some $s_0 \in \{1,...,m_0\}$.  We can assume that $\Sigma^0$ is in good position with $T_1^0, ..., T_{n_0}^0$. Then by Lemma 6.11, we can build new maximal nonparallel pairwise transverse tori $T_1^1, ..., T_{n_1}^1$ from $T_1^0, ..., T_{n_0}^0, \Sigma^0$ such that they satisfy the following conditions.
  \begin{itemize}
    \item $T_1^1, ..., T_{n_1}^1$  cuts   $M$ to $M_1^1, ..., M_{m_1}^1$, the maximal invariant set of $X|M_i^1$ ($i=1,...,m_1$) is denoted by $\Lambda_i^1$. $\Lambda_1^1 \cup ...\cup \Lambda_{m_1}^1$ just is the nonwandering set of $X|_{M-T_1^0 \cup ...\cup T_{n_0}^0 \cup \Sigma^0}$.
    \item $T_1^1 \cap \Lambda_{s_0}^0 \neq \emptyset$. Since periodic orbits are dense in $\Lambda_{s_0}^0$, there exists a periodic orbit $\gamma_0 \subset \Lambda_{s_0}^0$ such that $\gamma_0 \cap T_1^0 =\emptyset$ and $T_1^1 \cap \gamma_0 \neq \emptyset$.
    \item  Each $\Lambda_i^1 \subset \Lambda_{j_i}^0$ for some $j_i \in \{1,...,m_0\}$.
  \end{itemize}


By our supposition, this process can go on infinitely many steps. More precisely, for each $k\geq 0$, we have  maximal nonparallel, pairwise disjoint, transverse tori $T_1^k, ..., T_{n_k}^k$ which cut $M$ to $M_1^k, ..., M_{m_k}^k$ and the maximal invariant set of $X|M_i^k$ ($i\in \{1,...,m_k\}$) is denoted by $\Lambda_i^k$. There exists a transverse torus  $\Sigma^k$ which satisfies $\Sigma^{k+1} \cap \Lambda_{s_k}^k \neq \emptyset$ for some $s_k \in \{1,...,m_k\}$. Then by Lemma 6.11, we can build new  maximal nonparallel pairwise transverse tori $T_1^{k+1}, ..., T_{n_{k+1}}^{k+1}$ which satisfies the following conditions.
\begin{itemize}
    \item $T_1^{k+1}, ..., T_{n_{k+1}}^{k+1}$  cuts   $M$ to $M_1^{k+1}, ..., M_{m_{k+1}}^{k+1}$, the maximal invariant set of $X|M_i^{k+1}$ ($i=1,...,m_{k+1}$) is denoted by $\Lambda_i^{k+1}$. $\Lambda_1^{k+1} \cup ...\cup \Lambda_{m_{k+1}}^{k+1}$ just is the nonwandering set of $X|_{M-T_1^k \cup ...\cup T_{n_k}^k \cup \Sigma^k}$.
    \item $T_1^{k+1} \cap \Lambda_{s_k}^k \neq \emptyset$. Since periodic orbits are dense in $\Lambda_{s_k}^k$, there exists a periodic orbit $\gamma_k \subset \Lambda_{s_k}^k$ such that  $T_1^{k+1} \cap \gamma_k \neq \emptyset$.
    \item  Each $\Lambda_i^{k+1} \subset \Lambda_{j_i}^k$ for some $j_i \in \{1,...,m_k\}$.
  \end{itemize}





In the end,  we will use cohomology $H^i(M)=H^i(M,Q)$ to obtain a contradiction. By Poincare duality, every periodic orbit $\gamma$ of $X$ is corresponding to $[ \gamma] \in H^1(M)$, every embedded torus $T$ of $M$ is corresponding to $[T] \in H^2 (M)$  and $M$ (with a given orientation)
is corresponding to a generator of $H^3 (M)$: $[M]$. We denote the algebraic intersection number of $\gamma$ and $T$ by $int(\gamma, T)$. A standard theorem in homology theory tell us that the cup product of $[\gamma]$ and $[T]$ satisfies $[\gamma] \vee [T] = int(\gamma,T) [M]$.

For every $k\geq 0$,  periodic orbit $\gamma_k$ satisfies the following conditions.
\begin{itemize}
  \item $\gamma_k \cap (T_1^0\cup T_1^1\cup ...\cup T_1^k) =\emptyset$ since  for each $s\in \{0,1,..., k\}$, $\gamma_k \subset \Lambda_{j_s}^s$ for some $j_s \in \{1,...,m_s\} $

   \item $T_1^{k+1} \cap \gamma_k \neq \emptyset$.
\end{itemize}
So, $int (\gamma_k, T_1^i)=0$ for every $i\in \{0,1,...,k\}$. On the other hand, since   $T_1^{k+1}$ is a transverse torus, $int (\gamma_k, T_1^{k+1})$  is equal to the geometric intersection number of $T_1^{k+1}$ and $\gamma_k$. Moveover, since $T_1^{k+1} \cap \gamma_k \neq \emptyset$,
$int (\gamma_k, T_1^{k+1})\neq 0$.  This means $[\gamma_k] \vee [T_1^{k+1}]\neq 0$  and $[\gamma_k]\vee [T_1^i]=0$ for every $i\in \{0,1,...,k\}$.
Notice that $H^2(M)$ is a linear space, therefore $[T_1^{k+1}]$ can't be generated by $[T_1^0],[T_1^1],...,[T_1^k]$. This means the dimension of $H^2(M)$
is infinite. This conflicts to the fact that if $M$ is a closed 3-manifold, then $H^2(M)$  is a finite dimension linear space.

Therefore, there exists maximal nonparallel, pairwise disjoint transverse tori $T_1, ..., T_n$ which cut   $M$ to $M_1, ..., M_m$ and the maximal invariant set of $X|M_i$ is denoted by $\Lambda_i$ (obviously each $\Lambda_i$ is a basic set) which satisfies that, for every transverse torus $T$ of $X$ on $M$, $T\cap (\Lambda_1 \cup ... \cup \Lambda_m)=\emptyset$. Since $\Lambda_1 \cup ...\cup \Lambda_m$ is the closure of the periodic orbits set $\Gamma = \{\gamma\}$ here $\gamma$ is a periodic orbit of $X$ which doesn't intersect any transverse torus, they are unique.  Since a transverse torus of $X$ is incompressible (\cite{Br},\cite{Fe}), it is obviously that  $n\leq H(M)$ and $m\leq H(M)+1$ by the definition  of  Haken number $H(M)$.
\end{proof}

\begin{remark}
\begin{itemize}
  \item If $X$ is topologically equivalent to  a suspension of an Anosov diffeomorphism on $T^2$, transverse torus is unique up to flow-isotopy. This case belongs to a special case of the theorem: $m=0$.
  \item The transverse tori set of X which cut $M$ to filtrating neighborhoods of $\Lambda_1, ..., \Lambda_m$ always are not unique up to isotopy.    See Example ... .
\end{itemize}
\end{remark}

\begin{definition}
Let $X$ be an Anosov vector field on a closed orientable 3-manifold $M$ with transverse tori.  The series of  transitive, compact invariant sets $\Lambda_1, ..., \Lambda_m$ in Theorem .. is called \emph{spectrum like decomposition} of $X$.
\end{definition}


\begin{corollary}
Let $X$ be an Anosov vector field on a closed orientable 3-manifold $M$ with transverse tori. The spectrum like decomposition $\Lambda_1, ..., \Lambda_m$ of $X$ is minimal in the following sense. Suppose $T_1', ..., T_k'$ are maximal nonparallel, pairwise disjoint transverse tori  which cut   $M$ to $M_1', ..., M_r'$ and the maximal invariant set of $X|M_i'$ ($i\in\{1,...,r\}$) is denoted by $\Lambda_i'$ which is a transitive compact invariant set of $X$. Then for every $\Lambda_i$ ($i\in\{1,...,m\}$), there exists a $\Lambda_{j_i}'$ ($j_i \in \{1,...,r\}$) which satisfies $\Lambda_i \subset \Lambda_{j_i}'$.
\end{corollary}
\begin{proof}
It follows directly from the following facts.
\begin{enumerate}
  \item $\Lambda_1 \cup ...\cup \Lambda_m$ is the closure of the periodic orbits set $\Gamma = \{\gamma\}$ here $\gamma$ is a periodic orbit of $X$ which doesn't intersect any transverse torus.
  \item $\Lambda_1' \cup ...\cup \Lambda_r'$ is the closure of the periodic orbits set $\Gamma' = \{\gamma'\}$ here $\gamma'$ is a periodic orbit of $X$ which doesn't intersect $T_1' \cup ...\cup T_k'$.
  \item Both of $\Lambda_i$ and $\Lambda_j'$ are transitive compact invariant sets.
\end{enumerate}

\end{proof}


\subsection{DA order}
We call \emph{simple basic sets} the basic set whose \emph{model} have simple stable lamination on each connected component of the entrance.

We define a quantity for an irreducible manifold $M$ as the triple $(\|M\|, n(M), s(M))$ of real numbers, where
 \begin{enumerate}
   \item $\|M\|$ is Gromov's norm (i.e. the sum of the volumes of the hyperbolic pieces in the JSJ decomposition of $M$)
   \item $n(M)$ is the number of tori in the JSJ decomposition of $M$
   \item  $s(M)$ is the sum of the $-\chi(S)$ for each Seifert piece of the decomposition with some base surface S.
 \end{enumerate}

 Triples $(\|M\|, n(M), s(M))$ are ordered lexicographically. Notice that Gromov norms of 3-manifolds form a well-ordered set.

\begin{lemma}
Let $M$ be a closed orientable irreducible 3-manifold and $T_1,...,T_m$ be $m$ (nonparallel ?) pairwise disjoint incompressible tori in $M$ which bound a open 3-manifold $M_1^0 \subset M$. By a natural compactification of $M_1^0$, we obtain a compact 3-manifold $M_1^1$ with $n$ tori boundary $\Sigma_1, ..., \Sigma_n$. If we glue $n$ solid tori to $M_1^1$ along $\partial M_1^1$ such that we obtain a new closed orientable irreducible 3-manifold $M_1$, then $(\|M_1\|, n(M_1), s(M_1))<(\|M\|, n(M), s(M))$.
\end{lemma}



\begin{proof}
If some tori in $\{T_1,...,T_m\}$ are adjacent to some hyperbolic pieces of $\subset M$, by the construction of $M_1$ and Thurston's Dehn filling theorem, $\|M_1\| < \|M\|$.

If  there doesn't exist a torus in  $\{T_1,...,T_m\}$ is adjacent to some hyperbolic piece of $\subset M$ and there exists a torus $T_i \in \{T_1,...,T_m\}$ is isotopic to a JSJ torus of $M$, then $(\|M_1\|, n(M_1), s(M_1))<(\|M\|, n(M), s(M))$ since $\|M_1\|\leq \|M\|$ and $n(M_1)<
n(M)$.

Now, it remains to consider the case each $T_i$ ($i=1,...,m$) is a torus inside a Seifert piece and is not isotopic to any JSJ torus of $M$.
Because of this condition and the fact that $T_1,...,T_m$ are pairwise disjoint incompressible tori in $M$,  $s(M_1^1)< s(M)$.
Since $M_1$ is irreducible, the meridian of the Dehn filled tori can not be fiber-parallel. Therefore, if we regard that $M_1^1 \subset M_1$, the JSJ tori of $M_1$ and $M_1^1$ can be regarded as the same and $s(M_1)=s(M_1^1)< s(M)$.   On the other hand, it is easy to show that $\|M_1\| \neq \|M\|$ and $n(M_1)\neq n(M)$. In summery, $(\|M_1\|, n(M_1), s(M_1))<(\|M\|, n(M), s(M))$.
\end{proof}

\begin{proof} [Proof of Theorem~\ref{t.DAorder}]
By the definition of the order, $Y\prec_{DA} X$ means that some $DA$-bifurcation of $Y$ on a 3-manifold $N$ is a basic piece of the decomposition of $X$ on a 3-manifold $M$. It easy to see that in topology, constructing $N$ from $M$ just  is  the same proceed as constructing $M_1$ from $M$ in the condition of Lemma .. 3. Therefore, $(\|M_1\|, n(M_1), s(M_1))<(\|M\|, n(M), s(M))$. So, the relation $\prec_{DA}$ defined above is a (partial) order on the class of topological equivalence of Anosov flow on closed orientable $3$-manifolds.

Notice that $n(M), s(M)\in Z^+$ and Gromov norms of 3-manifolds form a well-ordered set \cite{Ma}, therefore the height $h(X)$ of every flow $X$ is finite.
\end{proof}

\subsection{Manifolds with several Anosov flows}
It is easy to obtain the following lemma as a corollary of Theorem 2 of the paper \cite{MaSm}.
\begin{lemma}
For a given $n\in N$, there exists a closed orientbale surface $\Sigma$ such that there exists a pseudo-Anosov diffeomorphism
$f$ on $\Sigma$ with an $n$-prong singularity.
\end{lemma}

 \begin{proof} [Proof of Theorem~\ref{t.manyanosov}]
  By Lemma ..., we have a pseudo-Anosov diffeomorphism $f$ on a closed orientable surface $\Sigma$ with a $2n+2$-prong singularity. Suppose $P_1,...,P_m$ are all singularities of $f$ and $P_1$ is an $n$-prong singularity. Now we can obtain a new diffeomorphism $g$ by  doing  DPA (derived from pseudo-Anosov) surgeries along
  $P_1,...,P_m$ such that the nonwandering set of $g$, $\Omega(g)$ is composed of a repeller $P_1$, $m-1$ attractors $P_2, ...,P_m$ and a transitive saddle invariant set $\Lambda_0$.

  Set $M_0= \Sigma \times [0,1]/(x,0)\sim (g(x),1)$ with a smooth vector field $Y=(\cdot, \frac{\partial}{\partial t})$. We denote $\gamma_i$ ($i=1,...,m$) to be the periodic orbit corresponding to $P_i$ and $\Lambda$ to be orbit of $\Lambda_0$. Obviously, $\Omega(Y)$ is composed of
  a repeller $\gamma_1$, $m-1$ attractors $\gamma_2, ...,\gamma_m$ and a transitive saddle invariant set $\Lambda$.  After cutting a small tubular neighborhoods of $\gamma_1, ..., \gamma_m$, we obtain a simple hyperbolic plug $U$ with vector field $Y|_U$. $\partial^{in} U \cap W^s (\Lambda)$
  provides $\partial^{in} U$ a foliation which is composed of $2n+2$ Reeb annuli. We define $T_1$ to be $\partial^{in} U$.  $\partial^{out} U$ is composed of $m-1$ tori $T_2,..., T_m$ and $W^u (\Lambda)$ provides each $T_i$ ($i=2,...,m$) a lamination  which always can be extended to a foliation composed of some Reeb annuli. By a well-known theorem of W. Thurston ([...]),  the interior of  $U$ is a hyperbolic manifold.

  Now we glue a filtrating neighborhood of a twisted periodic orbit $\gamma$, $V_4$ to $M_0$ along $\partial^{out} V_4$ and $\partial^{in} U$ such that $W^u (\gamma)\cap \partial^{in} U$ is a simple closed curve $c$ which is transverse to the lamination $W^s (\Lambda) \cap \partial^{in} U$ and is  in the interior of an annulus component of $W^s (\Lambda) \cap \partial^{in} U$.  Now $U$ and $V_4$ form a new simple hyperbolic plug $U_1$ with maximal invariant set $\Lambda_1$. Similar to ..., if we choose a good orientation, $W^s (\Lambda_1)$ can be extended to a foliation on $\partial^{in} U_1$ which is composed of $2n+1$ Reeb annuli and two adjacent suspension annuli with suitable orientation (see Figure ...).
  
  \begin{figure}[htp]
\begin{center}
  \includegraphics[totalheight=3.7cm]{figure6.eps}\\
  \caption{}\label{figure6}
  \end{center}
\end{figure}

  We continue to glue a copy of $V_4$ (which is called $\overline{V_4}$ and the corresponding periodic orbit is called $\overline{\gamma}$) to $U_1$ along $\partial^{out} \overline{V_4}$ and $\partial^{in} U$ such that $W^u (\overline{\gamma})\cap \partial^{in} U_1$ is a simple closed curve $c_1$ which is transverse to the lamination $W^s (\overline{\Lambda_1}) \cap \partial^{in} U_1$ and is  in the interior of the $k$ ($k\in \{1,...,n\}$) Reeb annulus of $W^s (\Lambda) \cap \partial^{in} U$. After this, we obtain a simple hyperbolic plug $W$ with maximal invariant set $\Lambda_0$. Again if we choose suitable orientation for the gluing, $W^s (\Lambda_1)$ can be extended to a foliation on $\partial^{in} W$ which is composed of $2n$ Reeb annuli and four adjacent suspension annuli $A_1^1$, $A_2^1$, $A_1^2$ and $A_2^2$ with suitable orientation such that $A_1^i$ and $A_2^i$ $i\in \{1,2\}$ are adjacent.  Denote the annulus composed of $A_1^i$ and $A_2^i$ ($i\in \{1,2\}$) by $B_i$.  $\overline{\partial^{in} W- (B_1 \cup B_2)}$ has two connected component: one is composed of $k$ Reeb annuli; the other is composed of $2n-k$ Reeb annuli.

   Let $\overline{U}$ be $U$ with converse vector field and $\overline{\Lambda}$ be the maximal invariant set in $\overline{U}$.  We glue $W$ to $\overline{U}$ under the following restrictions.
   \begin{itemize}
     \item $\partial^{in} W$ is attached to $\partial^{out} \overline{U}$.
     \item $\partial^{out} W$ is attached to $\partial^{in} \overline{U}$ such that the corresponding connected components are attached together.
     \item In $\partial^{in} W$, $W^s (\Lambda_1)$ and $W^u (\Lambda)$  transversely intersect. Similarly, in $\partial^{out} W$, $W^u (\Lambda_1)$ and $W^s (\Lambda)$  transversely intersect.
   \end{itemize}
  After gluing, we obtain a closed orientable 3-manifold $M$ with vector field $X_k$. By Theorem ..., $X_k$ is a transitive Anosov flow on $M$.
  For every two different integers  $i,j\in \{1,...,n\}$, we have two transitive Anosov flows $X_i$ and $X_j$ on $M$. The reason that $X_i$ and $X_j$ are on the same manifold $M$ is because of the fact that the gluing maps are in the same isotopic class of the corresponding tori.

   For finishing the proof of the theorem, we  have to check that $X_i$ and $X_j$ are homotopic and $X_i$ and $X_j$ are not topologically equivalent. The statement $X_i$ and $X_j$ are homotopic is easy followed from the facts that the smallest gluing pieces of $X_i$ and $X_j$ are the same  and the gluing maps are in the same isotopic class of the corresponding tori.

   The JSJ tori of $M$ are composed of $\partial^{out} W= \partial^{in} \overline{U}$, $\partial^{in} U = \partial^{out} V_2$ and $\partial^{in} \overline{V_2} =\partial^{out} \overline{U}$. We call them $\{T_2,...,T_m\}$, $T_1$ and $\overline {T_1}$ correspondingly. The corresponding JSJ
   pieces are $U$, $V_2 \cup \overline{V_2}$, $\overline{U}$ here $U$ and $\overline{U}$ are two hyperbolic pieces and $V_2 \cup \overline{V_2}$ is a Seifert piece.

   Suppose that there exist two different $i,j \in \{1,...,n\}$ such that $X_i$ is topologically equivalent to $X_j$, then there exists a self-homeomorphism $f$ on $M$ such that $f$ preserve  flowlines and the orientations of the flowlines. Obviously, $f$ maps JSJ tori to themselves. Since each of $T_1$ and $\overline {T_1}$ is adjacent to a hyperbolic piece (JSJ piece) and a Seifert piece but each $T_i$ ($i\in \{2,...,m\}$) is adjacent to two hyperbolic pieces, $f(T_1)$ is  isotopic to either $T_1$ or $\overline {T_1}$. Furthermore, since $f$ preserve the orientations of the flowlines, the unique possibility is that $f(T_1)$ is  isotopic to  $T_1$ and $f(\overline{T_1})$ is isotopic to $\overline{T_1}$.
   We denote the maximal invariant set of $(W,X_i |)$ and $(W, X_j |)$ by $\Lambda_2^i$ and $\Lambda_2^j$ correspondingly.
   Obviously, $f(\Lambda_2^i)$ is the maximal invariant set of $X_2$ restricting to $f(W)$ and up to leaf conjugacy, $W^s (\Lambda_2^i)\cap \partial^{in} W$ and $W^s (f(\Lambda_2^i))\cap \partial^{in} f(W)$
can be extended to the same foliation on a torus. On the other side, since  $f(W)$ is isotopic to $W$, $f(T_1)$ is isotopic to $T_1$ and $f(T_2 \cup ... \cup T_m)$ is isotopic to $T_2 \cup...\cup T_m$, by Lemma 6.13, it is easy to show $(f(W), X_j |)$ is topologically equivalent to $(W,X_j |)$. Therefore,   $W^s (f(\Lambda_2^i))\cap \partial^{in} W$ and $W^s (\Lambda_2^j)\cap \partial^{in} W$ can be extended to the same foliation in a torus. Recall the meaning of $i$ and $j$, it tells us that $W^s (\Lambda_2^i)$  and $W^s (\Lambda_2^j)$ can't be extended to the same foliation on a torus. It is a contradiction. Therefore, $X_i$ and $X_j$ are not topologically equivalent.
\end{proof}



